PGAbB: A Block-Based Graph Processing Framework for Heterogeneous Platforms

Designing flexible graph kernels that can run well on various platforms is a crucial research problem due to the frequent usage of graphs for modeling data and recent architectural advances and variety. In this work, we propose a novel graph processing framework, PGAbB (Parallel Graph Algorithms by Blocks), for modern shared-memory heterogeneous platforms. Our framework implements a block-based programming model. This allows a user to express a graph algorithm using kernels that operate on subgraphs. PGAbB support graph computations that fit in host DRAM but not in GPU device memory, and provides simple but effective scheduling techniques to schedule computations to all available resources in a heterogeneous architecture. We have demonstrated that one can easily implement a diverse set of graph algorithms in our framework by developing five algorithms. Our experimental results show that PGAbB implementations achieve better or competitive performance compared to hand-optimized implementations. Based on our experiments on five graph algorithms and forty-four graphs, in the median, PGAbB achieves 1.6, 1.6, 5.7, 3.4, 4.5, and 2.4 times better performance than GAPBS, Galois, Ligra, LAGraph Galois-GPU, and Gunrock graph processing systems, respectively.

==> Makefile <==
PAPER = paper
VERBOSE = 0

# directories
FIGURE_DIR = ./figures
OUTPUT_DIR = ./
STYLE_DIR = ./
TEXT_DIR = ./
BIB_OUT_FILE = $(OUTPUT_DIR)/bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR)/sty:$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(OUTPUT_DIR)/$(PAPER).log | sed -n '1h;1!H;$${;g;s/\n / /g;p;}' | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat $(OUTPUT_DIR)/*.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)

#formats
NORM=
BOLD=
PS2PDF_LABEL   =[ps2pdf   ]
DVIPS_LABEL    =[dvips    ]
LATEX_LABEL    =[pdflatex ]
BIBTEX_LABEL   =[bibtex   ]
NOTE_LABEL     =[note     ]
MAKEINDEX_LABEL=[makeindex]
RM_LABEL       =[rm       ]

SHELL:=/bin/bash

all: $(OUTPUT_DIR)/$(PAPER).pdf

show: $(OUTPUT_DIR)/$(PAPER).pdf
	@open $(OUTPUT_DIR)/$(PAPER).pdf &

$(OUTPUT_DIR)/$(PAPER).pdf: $(TEXT_DIR)/$(PAPER).tex                     \
                           $(shell find $(TEXT_DIR) -regex "[^.]*.tex")  \
                           $(shell find $(TEXT_DIR) -regex  "[^.]*.bib") \
                           $(shell find $(STYLE_DIR) -regex "[^.]*.tex") \
                           $(shell find $(FIGURE_DIR) -name "*.pdf")
	@mkdir -p $(OUTPUT_DIR)

	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS) $(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi
	@-$(PRINT_BIBTEX_WARNINGS)
	@echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."

#	@echo "$(MAKEINDEX_LABEL)Building index..."
#	@makeindex $(MAKEINDEX_OPTS) $(OUTPUT_DIR)/$(PAPER).idx || \
#		(rm -f $@ && exit 1)

	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

#	@echo "$(LATEX_LABEL)Performing ternary latex..."
#	@TEXINPUTS=$(TEX_PATH) \
#		latex $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
#			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)

clean:
	@echo '$(RM_LABEL)Cleaning project...'
	@rm  $(OUTPUT_DIR)/paper.pdf \
		$(OUTPUT_DIR)/paper.log \
		$(OUTPUT_DIR)/paper.aux \
		$(OUTPUT_DIR)/paper.bbl \
		$(OUTPUT_DIR)/paper.blg \
		$(OUTPUT_DIR)/bib-issues
